Two-pion femtoscopic correlations in Be+Be collisions at $\sqrt{s_{\textrm{NN}}} = 16.84$ GeV measured by the NA61/SHINE at CERN

This paper reports measurements of two-pion Bose-Einstein (HBT) correlations in Be+Be collisions at a beam momentum of 150$A\,\mbox{GeV}/\textit{c}$ by the $\mbox{NA61/SHINE}$ experiment at the CERN SPS accelerator. The obtained momentum space correlation functions can be well described by a L\'evy distributed source model. The transverse mass dependence of the L\'evy source parameters is presented, and their possible theoretical interpretations are discussed. The results show that the L\'evy exponent $\alpha$ is approximately constant as a function of $m_{\rm{T}}$ , and far from both the Gaussian case of $\alpha = 2$ or the conjectured value at the critical endpoint, $\alpha = 0.5$. The radius scale parameter $R$ shows a slight decrease in $m_{\rm{T}}$, which can be explained as a signature of transverse flow. Finally, an approximately constant trend of the intercept parameter $\lambda$ as a function of $m_{\rm{T}}$ was observed, different from measurement results at RHIC.

==> Makefile <==
# $Id: Makefile 3210 2013-10-26 17:12:15Z darko $

USEPDFLATEX := 1
USEBIBTEX := 0

TARGET := na61_revtex4_template

##########################################################

LATEX := $(if $(filter 1, $(USEPDFLATEX)), pdflatex, latex)

COLORIZE := awk 'BEGIN{red="\033[31;1m";yel="\033[34m";byel="\033[34;1m";end="\033[0m"}/Rerun /||/rerunfilecheck[^.]/{e=e$$0"\n";print red""$$0""end;next}/^LaTeX Warning:/||/natbib Warning:/{w=w$$0"\n";print yel""$$0""end;next}{print}END{if(w||e)print "\n"red"Warning/error summary:\n"byel""w""end;if(e){print red""e""end;exit 1}}'

define basic_latex_rule
  for i in 1 2 3 ; do $(LATEX) $< | $(COLORIZE) && break ; done
endef

ifeq ($(USEBIBTEX), 1)
define latex_rule
  $(LATEX) $< ; bibtex $*
  $(call basic_latex_rule)
endef
else
define latex_rule
  $(call basic_latex_rule)
endef
endif

.PHONY: all clean distclean

all: $(TARGET).tex $(TARGET).pdf $(TARGET).ps

na61_revtex4_template.tex: ../db/author_list.xml
	../generate.pl -t revtex4 -f $^ >$@

# dependencies
$(TARGET).pdf: $(DEPENDENCIES)

clean:
	- for e in .tex~ .ps .pdf .dvi .log .aux .toc .nav .out .snm .bbl .blg .spl .lof Notes.bib .maf .fff .lot .ttt ; do rm -f $(TARGET)$$e ; done

distclean: clean
	- rm -f $(TARGET).tex

# general rules
ifeq ($(USEPDFLATEX), 1)
%.pdf %.dvi: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.ps: %.pdf
	pdf2ps $<
else
%.dvi: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.pdf: %.ps
	ps2pdf $<

%.ps: %.dvi
	dvips $< -o
endif


==> na61AuthorsLimited.tex <==
% based on XML DB with time Thu Jan 26 09:03:08 2023
% Authors in alphabetical order.

\noindent
S.~Bordoni$^{\,6}$,
A.~Bravar$^{\,5}$,
N.~Charitonidis$^{\,6}$,
P.~Christakoglou$^{\,1}$,
G.~Christodoulou$^{\,6}$,
A.~De~Roeck$^{\,6}$,
F.~Diakonos$^{\,1}$,
S.J.~Dolan$^{\,6}$,
R.A.~Fernandez$^{\,6}$,
K.J.~Floethner$^{\,6}$,
A.~Kapoyannis$^{\,1}$,
U.~Kose$^{\,6}$,
M.O.~Kuttan$^{\,3}$,
O.~Linnyk$^{\,3}$,
W.C.~Louis$^{\,2}$,
L.~Munteanu$^{\,6}$,
C.~Mussolini$^{\,6}$,
A.D.~Panagiotou$^{\,1}$,
J.~Pawlowski$^{\,3}$,
W.~Rauch$^{\,4}$,
L.~Scharenberg$^{\,6}$,
S.~Schramm$^{\,3}$,
J.~Steinheimer-Froschauer$^{\,3}$,
H.~Stoecker$^{\,3}$,
M.~Vassiliou$^{\,1}$,
C.F.~Vilela$^{\,6}$, and
K.~Zhou$^{\,3}$


==> na61InstitutionsLimited.tex <==
% based on XML DB with time Thu Jan 26 09:03:08 2023
% Institutes in alphabetical order.

\noindent
$^{1}$~University of Athens, Athens, Greece\\
$^{2}$~Los Alamos National Laboratory, USA\\
$^{3}$~Frankfurt Institute for Advanced Studies, Frankfurt, Germany\\
$^{4}$~Fachhochschule Frankfurt, Frankfurt, Germany\\
$^{5}$~University of Geneva, Geneva, Switzerland\\
$^{6}$~CERN, Geneva, Switzerland\\

